Probabilistic Scan Matching: Bayesian Pose Estimation from Point Clouds

Estimating position and orientation change of a mobile platform from two consecutive point clouds provided by a high-resolution sensor is a key problem in autonomous navigation. In particular, scan matching algorithms aim to find the translation and rotation of the platform such that the two point clouds coincide. The association of measurements in point cloud one with measurements in point cloud two is a problem inherent to scan matching. Existing methods perform non-probabilistic data association, i.e., they assume a single association hypothesis. This leads to overconfident pose estimates and reduced estimation accuracy in ambiguous environments. Our probabilistic scan matching approach addresses this issue by considering all association hypotheses with their respective likelihoods. We formulate a holistic Bayesian estimation problem for both data association and pose estimation and present the corresponding joint factor graph. Near-optimum maximum a posteriori (MAP) estimates of the sensor pose are computed by performing iterative message passing on the factor graph. Our numerical study shows performance improvements compared to non-probabilistic scan matching methods that are based on the normal distributions transform (NDT) and implicit moving least squares (IMLS).

==> Figures/factorGraph/factorGraph.tex <==
\psfrag{pose}[cc][cc][.85][0]{Pose Estimation Layer}
\psfrag{ass}[cc][cc][.85][0]{Data Association Layer}
\psfrag{fp}[c][][.85][0]{$f_{\Delta\M{P}}$}
\psfrag{fn}[c][][.85][0]{$v_{\mathrm{NA}}$}
\psfrag{dp}[c][][.85][0]{$\Delta\M{P}$}
\psfrag{q1}[c][][.85][0]{$q_1$}
\psfrag{qN}[c][][.85][0]{$q_{N_{\mathrm{D}}}$}
\psfrag{a1}[c][][.85][0]{$a^{(1)}$}
\psfrag{aN}[c][][.85][0]{$a^{(N_{\mathrm{D}})}$}
\psfrag{b1}[c][][.85][0]{$b^{(1)}$}
\psfrag{bN}[c][][.85][0]{$b^{(N_{\mathrm{S}})}$}
\psfrag{mufpp}[c][][.85][0]{$\mu_{f_{\Delta\M{P}} \rightarrow \Delta\M{P} }$}
\psfrag{psi11}[c][][.75][0]{$\psi_{1,1}$}
\psfrag{psi1N}[c][][.75][0]{$\psi_{1,N_{\mathrm{S}}}$}
\psfrag{psiN1}[c][][.75][0]{$\psi_{N_{\mathrm{D}},1}$}
\psfrag{psiNN}[c][][.75][0]{$\psi_{N_{\mathrm{D}},N_{\mathrm{S}}}$}


==> Figures/scenario/scenario.tex <==
\psfrag{p1}[lc][lc][.85][0]{$\M{P}_{\mathrm{s}}$}
\psfrag{p2}[lc][lc][.85][0]{$\M{P}_{\mathrm{d}}$}
\psfrag{dp}[lc][lc][.85][0]{$\Delta\M{P}$}
\psfrag{s1}[lc][lc][.85][0]{\color[rgb]{0.1137,    0.5882,    0.6078}{$\V{s}^{(1)}$}}
\psfrag{s2}[lc][lc][.85][0]{\color[rgb]{0.1137,    0.5882,    0.6078}{$\V{s}^{(2)}$}}
\psfrag{sN}[lc][lc][.85][0]{\color[rgb]{0.1137,    0.5882,    0.6078}{$\V{s}^{(N_{\mathrm{\mathrm{S}}})}$}}
\psfrag{d1}[lc][lc][.85][0]{\color[rgb]{0.8471,    0.2157,    0.5647}{$\V{d}^{(1)}$}}
\psfrag{d2}[lc][lc][.85][0]{\color[rgb]{0.8471,    0.2157,    0.5647}{$\V{d}^{(2)}$}}
\psfrag{dN}[lc][lc][.85][0]{\color[rgb]{0.8471,    0.2157,    0.5647}{$\V{d}^{(N_{\mathrm{\mathrm{D}}})}$}}
\psfrag{n1}[lc][lc][.85][0]{\color[rgb]{0.8471,    0.2157,    0.5647}{$\V{n}^{(1)}$}}
\psfrag{n2}[lc][lc][.85][0]{\color[rgb]{0.8471,    0.2157,    0.5647}{$\V{n}^{(2)}$}}
\psfrag{nN}[lc][lc][.85][0]{\color[rgb]{0.8471,    0.2157,    0.5647}{$\V{n}^{(N_{\mathrm{\mathrm{D}}})}$}}


==> Figures/urbanEnvironment/urbanEnvironmentCar.tex <==
\psfrag{gt}[lc][lc][.8][0]{Ground Truth}
\psfrag{pr}[lc][lc][.8][0]{Proposed}
\psfrag{imls}[lc][lc][.8][0]{IMLS [6]}
\psfrag{ndt}[lc][lc][.8][0]{NDT [3]}
\psfrag{scan}[lc][lc][.8][0]{Scan Points}
\psfrag{10}[lc][lc][.8][0]{10}
\psfrag{0}[lc][lc][.8][0]{0}
\psfrag{20}[lc][lc][.8][0]{20}
\psfrag{30}[lc][lc][.8][0]{30}
\psfrag{40}[lc][lc][.8][0]{40}
\psfrag{m10}[lc][lc][.8][0]{-10}
\psfrag{x}[lc][lc][.8][0]{Horizontal distance in m}
\psfrag{y}[lt][lc][.8][90]{Vertical distance in m}

==> paperOrganization.tex <==
%----------------------------------------------------------------------------------------%
%                                   Paper Organization                                  %
%----------------------------------------------------------------------------------------%
\section*{Research Paper Organization\footnote{Adapted from George Heilmeier.}} 

\vspace{0.5cm} 

\be\itemsep3ex

\item What is the big picture? What is the problem and why is it hard?
	\bi
	\item[$\diamond$] The Big Picture: \BigPicture
	\item[$\diamond$] The Problem/Difficulty: \ProblemDifficulty
%	\item[$\diamond$] The Difficulty:
	\ei

\item What are the classical approaches? What is the state-of-the-art and what are the deficiencies?
	\bi
	\item[$\diamond$] Classical Approaches: \ClassicApproach
	\item[$\diamond$] The State-of-the-Art and Deficiencies:  \SOADeficiency
	\item[ ] \mysubsubnote{This is where you make a literature review. Articulate the deficiencies and shortcomings of previous work. Provide references (you can use the first three alphabets of the authors' last names and year, similar to the convention in our database).}
	\ei
	
\item What are the fundamental questions relevant to the problem? How answering to these questions can impact the design, architecture, and operation?
	\bi
	\item[$\circ$] \FundamentalQ
	\item[$\circ$] \EnablingA 
	\item[ ] \mysubsubnote{This is where you persuade the reader that these are fundamental questions, and the answers to these questions will have game-changing impacts.}
	\ei	

\item What are the goals of our paper?
	\bi
	\item[$\diamond$] The Goals:
	\item[ ] \mysubsubnote{Describe the goals at a high level; this should correlate with high-level contributions in Question 6.}
	\ei
		\be
		\item[$\circ$] \Goals 
		\ee		
\item What are we advocating; what is the new technical idea; what is our new view; what is our credence? Why we can succeed now? 
	\bi
	\item[$\diamond$] Advocacy, Idea, View, and Credence:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \Advocacy 
		\ee
	\item[$\diamond$] Reasons for Success:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \ReasonSuccess 
		\ee
	\ei

\item What are the high-level contributions of our  paper? What are the key contributions of our paper? 
	\bi
	\item[$\diamond$] High-Level Contributions: \HLContribution
	\item[ ] \mysubsubnote{Describe what we do at a high level; this should address the goal that we set out in Question 4; for example:}
		\be
		\item[$\circ$] In this paper, \ldots
		\ee
	\item[$\diamond$] Key Contributions:
	\item[ ] \mysubsubnote{Provide a bulletized list (usually 3-5 bullets, equal number of lines per bullets); for example:}
		\be
		\item[$\circ$] \KeyContribution
		\ee
	\ei


\item Which are the methodologies (analysis, simulation, experimentation, heterogeneous approach) used in this paper? How is the approach verified; how are the results confirmed?
	\bi
	\item[$\diamond$] The Methodologies:
	\item[$\diamond$] The Verification:
	\ei
	
\item What are the new vision/perspective we provide? What are the lessons learned?
	\bi
	\item[$\diamond$] The New Vision/Perspective: \ConclusiveVision
	\item[$\diamond$] The Lessons Learned/Surprising Results: \ConclusiveLesson
	\ei

\item What is the impact; what are the benefits or merits of the results to a broader community?
	\bi
	\item[$\diamond$] The Impact/Benefit: \Benefit
	\item[ ] \mysubsubnote{Think of strong conclusions for the paper when answering them}
	\ei


\item Where the known results appear in the paper?
	\bi
	\item[$\diamond$] Disclosures:
	\item[ ] \mysubsubnote{Identify where known results appear in the paper (point to specific section numbers before the paper is written; point to specific section, page, line, equation numbers, etc. after the paper is written).}
	\item[$\diamond$] Sources:
	\item[ ] \mysubsubnote{Identify what are the sources (provide reference, section, page, line, equation numbers, etc. of the sources).}
	\ei

\item What are the key references?
\bi
	\item[ ] \mysubsubnote{List the key references that we used to develop this paper (rather than the references for the state-of-the-art).}
\ei

\ee

